Observational Diagnostics of Self-Gravitating MHD Turbulence in Giant Molecular Clouds

We study the observable signatures of self-gravitating MHD turbulence by applying the probability density functions (PDFs) and the spatial density power spectrum to synthetic column density maps. We find that there exists three characterizable stages of the evolution of the collapsing cloud which we term "early," "intermediate," and "advanced." At early times, i.e. $t<0.15t_{ff}$, the column density has a power spectral slope similar to nongravitating supersonic turbulence and a lognormal distribution. At an intermediate stage, i.e. $0.15t_{ff}< t \leq 0.35t_{ff}$, there exists signatures of the prestellar cores in the shallower PDF and power spectrum power law slopes. The column density PDF power law tails at these times have line of sight averaged slopes ranging from -2.5 to -1.5 with shallower values belonging to simulations with lower magnetic field strength. The density power spectrum slope becomes shallow and can be characterized by $P(k)=A_1k^{\beta_2}e^{-k/k_c}$, where $A_1$ describes the amplitude, $k^{\beta_2}$ describes the classical power law behavior and the scale $k_c$ characterizes the turn over from turbulence dominated to self-gravity dominated. At advanced stages of collapse, i.e. $\approx t>0.35t_{ff}$, the power spectral slope is positive valued, and a dramatic increase is observed in the PDF moments and the Tsallis incremental PDF parameters, which gives rise to deviations between PDF-sonic Mach number relations. Finally, we show that the imprint of gravity on the density power spectrum can be replicated in non-gravitating turbulence by introducing a delta-function with amplitude equivalent to the maximum valued point in a given self-gravitating map. We find that the turbulence power spectrum restored through spatial filtering of the high density material.

==> go <==
#!/bin/csh
set echo
if ( 0 == 1 ) then 
set name = "ms"
set this_latex = latex

#pdflatex is better, but apj still wants the antiquated eps format.
#the pdftrue/pdffalse easily toggles between pdf/eps for papers.

if( `grep  "^\\pdftrue" ms.tex |wc -l` == 1 ) set this_latex = pdflatex
if( `grep  "^\\pdffalse" ms.tex |wc -l` == 1 ) set this_latex = latex

#I like the paper to open when I'm done.
#Sort out the extant program
if( -e /usr/bin/acroread ) then
 set run = "acroread"
else
 set run = "open"
endif    

#clean up stuff.
rm -f *.log *.out *.aux *.dvi *~ *.bbl *.blg
rm -f *.ps $name.pdf *.bak *.toc *.lof *.lot
set make_only = no
set clean_only = no
set no_open = no
set no_bib = no

#parse command line arguments.
while( $#argv )
  switch ( $1 )
    case "o":
      set make_only = "yes"
      shift 
      breaksw
    case "c":
      set clean_only = "yes"
      shift
      breaksw
    case "n":
      set no_open = "yes"
      shift
      breaksw
    case "nb":
      set no_bib = "yes"
      shift
      breaksw
    default:
      set name = $1
      shift
      breaksw
  endsw
end

if( $clean_only == "yes" ) then
    exit
endif

if( $make_only == "yes" ) then
    $this_latex $name
else
    
    $this_latex $name

    #check for errors
    if( $status != 0 ) then
      echo "done borked sompin. Exiting."
      exit
    endif

    if ( $no_bib != 'yes' ) then
      bibtex $name
      $this_latex $name
      $this_latex $name
      #I don't get why my current version of latex/bibtex is putting this junk
      #in my bbl file.  
      mv ms.bbl derp.bbl
      #egrep -v "REVTEX41Control|????|apsrev41Control|^08. 1" derp.bbl > ms.bbl
      egrep -v "^ \?\?\?\?|^08. 1" derp.bbl > ms.bbl
      $this_latex $name
    endif
    if( $no_open != 'yes' ) then
      #dvi to eps to pdf if necessary
      if( -e $name.dvi ) then
        dvips -Ppdf -t letter -o $name.ps $name.dvi
        ps2pdf $name.ps $name.pdf
  	    if( $status != 0 )then
  		    print "dvipdf borked.  That's *really* too bad."
          exit
  	    endif
  	  endif
  	  if(  -e $name.pdf && 0 == 1 ) $run $name.pdf &
    endif	    
endif
endif 
print no
latex ms
set name = ms
dvips -Ppdf -t letter -o $name.ps $name.dvi
ps2pdf $name.ps $name.pdf
# the end

